Additive Approximations in High Dimensional Nonparametric Regression via the SALSA

High dimensional nonparametric regression is an inherently difficult problem with known lower bounds depending exponentially in dimension. A popular strategy to alleviate this curse of dimensionality has been to use additive models of \emph{first order}, which model the regression function as a sum of independent functions on each dimension. Though useful in controlling the variance of the estimate, such models are often too restrictive in practical settings. Between non-additive models which often have large variance and first order additive models which have large bias, there has been little work to exploit the trade-off in the middle via additive models of intermediate order. In this work, we propose SALSA, which bridges this gap by allowing interactions between variables, but controls model capacity by limiting the order of interactions. SALSA minimises the residual sum of squares with squared RKHS norm penalties. Algorithmically, it can be viewed as Kernel Ridge Regression with an additive kernel. When the regression function is additive, the excess risk is only polynomial in dimension. Using the Girard-Newton formulae, we efficiently sum over a combinatorial number of terms in the additive expansion. Via a comparison on $15$ real datasets, we show that our method is competitive against $21$ other alternatives.

==> LCtableHash.tex <==

\newcommand{\insertTableReal}{
\newcommand{\tabletitlenumberspace}{-0.12in}
% \begin{sidewaystable}
\begin{landscape}
\begin{table}
{ %\footnotesize
\centering
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c}
% Dataset ($D$, $n$) & \addkrr & \krr & \ll & \lq & \svr & \gp & \backf  & \krr & \nw  \\
Dataset ($D$, $n$) & \addkrrs ($d$) & \krr & \knn & \nw & \locallin & \localquad 
  &\localcubic & \sveps &\svnu & \gp & \rt  \\
\hline \\[\tabletitlenumberspace]
\hline 

Housing ($12$, $256$)& $\bf{0.26241}$ (9) & $\underline{0.37690}$ & $0.43620$ & $0.38431$ & 
  $\underline{0.31219}$ &
$\underline{0.35061}$ & $0.38528$ & $1.15272$ & $0.38600$ & $0.67563$ 
& $1.06015$   \\ \hline
% % Indicate times here
% \emph{Training time} & $2.11 s$ & $0.18 s$ & $0.14 s$ & $0.65 s$ & $0.98 s$ &
% $1.54 s$ & $2.16 $& $0.20 s$ & $2.99 s$ & $1.67 s$  & $0.15 s$
% \\ \hline

Galaxy ($20$,$2000$)
& $\bf{0.00014}$ (4) & $0.01317$ & $0.25854$ & $0.30615$ & $0.01676$ & $0.00175$ &
$\underline{0.00076}$ & $0.65280$ & $0.15798$ & $0.00221$ & $0.02293$  \\ \hline

fMRI ($100$,$700$)
& $\bf{0.80730}$ (2) & $0.86495$ & $0.85645$ & $0.84989$ & $0.91098$ & $1.14079$ &
$1.85969$ & $\underline{0.81080}$ & $\underline{0.81376}$ & $0.84766$ & $1.52834$  \\ \hline

Insulin ($50$,$256$)
& $\bf{1.02062}$ (3) & $\underline{1.09023}$ & $1.15578$ & $1.18070$ & 
$\underline{1.06457}$ & $1.35747$ &
$1.35747$ & $1.10725$ & $\underline{1.09140}$ & $1.22404$ & $1.58009$  \\ \hline

Skillcraft ($18$,$1700$)
& $\bf{0.54695}$ (1) & $\underline{0.54803}$ & $0.67155$ & $0.73258$ & $0.60581$ & $1.29690$ &
$21.4205$ & $0.71261$ &
$0.66311$ & $\underline{0.54816}$ & $1.08047$  \\ \hline

Airfoil* ($40$,$750$)
& $\bf{0.48487}$ (5) & $\underline{0.50170}$ & $0.87755$ & $0.91717$ & $0.50549$ & $\bf{0.48020}$ &
$0.53177$& $0.62141$ & $0.64011$ & $0.74639$ & $\underline{0.50400}$  \\ \hline

School ($36$,$90$)
& $\underline{1.32008}$ (2) & $1.64315$ & $\underline{1.37910}$ & $\bf{1.14866}$ & 
$2.13390$ & $4.79447$ &
$88.361$ & $\underline{1.38173}$ & $1.48746$ & $1.64215$ & $1.99244$  \\ \hline

CCPP* ($59$,$2000$)
& $\underline{0.06782}$ (2) & $0.08038$ & $0.32017$ & $0.33863$ & $0.07568$ & 
  $\underline{0.06779}$ &
$\underline{0.06897}$ & $0.33707$ & $0.094493$ & $0.11128$ & $1.04527$  \\ \hline

% Dataset ($D$, $n$) & \addkrr & \krr & \knn & \nw & \locallin & \localquad 
%   &\localcubic & \sveps &\svnu & \gp & \rt & \rbfi \\

Blog ($91$,$700$)
& $\underline{1.42266}$ (4) & $\underline{1.42699}$ & $1.5351$ & $2.13129$ & $2.23489$ & 
$2.98756$ & $9.87324$ & $1.66705$ & $1.87561$ &
$1.64429$ & $\underline{1.41227}$  \\ \hline

Bleeding ($100$,$200$)
& $\underline{0.00123}$ (5) & $0.10633$ & $0.16727$ & $0.19284$ & $\bf{2.48\textrm{e}
-6}$ & $0.00614$ &
$47.113$ & $0.36505$ & $0.03168$ & $\underline{6.68\textrm{e}-6}$ & $0.18292$  \\ \hline


Speech ($21$, $520$)& $\underline{0.02246}$ (2) & $0.03036$ & $0.09348$ & $0.11207$ & 
$0.03373$ &
$\underline{0.02404}$ & $0.02412$ & $\underline{0.22431}$ & $0.06994$ & $0.02531$ & $0.05430$  \\
% Indicate times here
\hspace{0.3in}\emph{Training time} & $4.71 s$ & $0.8 s$ & $0.18 s$ & $1.81 s$ & $4.53 s$ &
$6.80 s$ & $9.94 s$& $0.24 s$ & $27.43 s$ & $6.34 s$  & $0.21 s$
\\ \hline

Music ($90$,$1000$)
& $\underline{0.62512}$ (3) & $\underline{0.61244}$ & $0.71141$ & $0.75225$ & $0.67271$ & $1.31957$ &
$3.80597$ & $0.75420$ & $\bf{0.59399}$ & $\underline{0.62429}$ & $1.45983$  \\ \hline

Telemonit ($19$, $1000$)
& $\underline{0.03473}$ (9) & $0.05640$ & $0.09262$ & $0.21198$ & $0.08253$ & $0.18399$ &
$99.958$ & $0.33902$ & $0.05246$ & $\underline{0.03948}$ & $\bf{0.01375}$ \\ \hline

Forestfires($10$, $211$)
& $\underline{0.35301}$ (3) & $\underline{0.28771}$ & $0.36571$ & $0.37199$ 
& $0.35462$ & $12.5727$ &
$179.469$ & $0.70154$ & $0.43142$ & $\underline{0.29038}$ & $0.41531$  \\ \hline

Propulsion ($15$,$200$) & $\underline{0.00881}$ (8) & $0.05010$ & $0.14614$ & $0.11237$ &
$1.12712$ &
$1.12801$ & $1.14312$ & $0.74511$ & $\underline{0.00910}$ & $\underline{0.00355}$ & $0.02341$   \\ \hline

Brain ($29$,$300$)
& $0.00036$ (2) & $0.01239$ & $0.24429$ & $0.22929$ & $1.23412$ & $2.45781$ &
$19.7543$ &
$0.27204$ & $0.05556$ & $\underline{5\textrm{e}-14}$ & $0.00796$  \\ \hline 
\hline \\[-0.06in]

% Dataset ($D$, $n$) & \addkrr & \krr & \knn & \nw & \locallin & \localquad 
%   &\localcubic & \sveps &\svnu & \gp & \rt & \rbfi \\

% \hline \\[-0.00in]
% \hline
  & \rbfi
 & \mfp & \si & \backf & \mars & \cosso & \spam &\addgp
  & \lr & \lasso & \lar  \\
\hline \\[\tabletitlenumberspace]
\hline 

Housing ($12$, $256$)& $0.64871$ & $\underline{0.38256}$ & $0.50445$ & $0.64218$ & $0.42379$ & $1.30965$ &
$0.81653$ & $0.45656$ & $95.60708$ & $0.44515$ & $0.84410$  \\ \hline
% % Indicate times here
% \emph{Training time} & $0.04 s$ & $0.49 s$ & $0.12 s$ & $6.30 s$ & $0.68 s$ &
% $1.74 s$ & $17.74 s$& $\sim 3\, mins$ & $0.01 s$ & $1.08 s$  & $0.06 s$
% \\ \hline

Galaxy ($20$,$2000$) & $0.01532$
& $\underline{0.00116}$ & $0.92189$ & $0.94165$ & $\underline{0.00163}$ 
& $\underline{0.00153}$ & $0.95415$ 
& $-$ & $0.13902$ & $0.02392$ & $1.02315$  \\ \hline

fMRI ($100$,$700$)
& $1.38585$ & $1.42795$ & $0.90595$ & $0.86197$ & $0.90850$ & $0.82448$ & $0.88014$ &
$-$&
$\underline{0.81005}$ & $\underline{0.81390}$ & $0.88351$  \\ \hline

Insulin ($50$,$256$)
& $1.22404$ 
& $1.78252$ & $1.20771$ & $1.16524$ & $1.10359$ & $1.13791$ & $1.20345$ & $-$
& $\bf{1.02051}$ &
$1.11034$ & $1.22404$  \\ \hline

Skillcraft ($18$,$1700$)
& $0.81966$ & $1.07195$ & $0.87677$ & $0.83733$ & $\bf{0.54595}$ &
$\underline{0.55514}$ & $0.905445$ &
$-$ & $0.70910$ & $0.66496$ & $1.00048$  \\ \hline

Airfoil* ($40$,$750$)
 & $1.00909$
& $0.51463$ & $0.99420$ & $0.96778$ & $0.51856$ & $\underline{0.50402}$ & $0.96267$ & $-$ & $0.51749$ &
$0.52159$ & $1.00910$  \\ \hline

School ($36$,$90$)
& $1.61927$ & $1.72657$ & $1.52374$ & $1.48866$ & $1.44453$ & $1.48046$ & $1.59328$ &
$-$ & $1.53416$ & $\underline{1.34467}$ & $1.64330$  \\ \hline

CCPP* ($59$,$2000$)
& $1.04257$ & $0.10513$ & $0.97223$ & $0.88084$ & $0.08189$ & $0.96844$ & $\bf{0.06469}$ &
$-$ & $0.07641$ & 
$\underline{0.07395}$ & $1.04527$  \\ \hline


Blog ($91$,$700$)
& $3.45781$ & $1.50871$  
& $1.98495$ & $1.45293$ & $1.68015$ & $1.96042$ & $1.94262$ & $-$ &
$\underline{1.43368}$
  & $\bf{1.22737}$ & $2.05927$
\\ \hline

Bleeding ($100$,$200$)
& $0.13872$ & $0.00210$ & $0.24918$ & $0.37840$ & $0.00497$ & $0.31362$ & $0.41735$ &
 $-$ & $\underline{0.00001}$ & $\underline{0.00191}$ & $0.43488$  \\ \hline


Speech ($21$, $520$)
& $0.03339$  
& $0.02843$ & $0.39883$ & $0.36793$ & $\bf{0.01647}$ & $0.34863$ &
$0.66009$ & $\underline{0.02310}$ & $0.07392$ & $0.07303$ & $0.73916$  \\
% Indicate times here
 \hspace{0.3in}\emph{Training time} & $0.12 s$ & $5.70 s$ & $0.66 s$ & $27.93 s$ & $8.11 s$ &
$9.40 s$ & $76.39 s$& $79\,mins$ & $0.03 s$ & $15.94 s$  & $0.06 s$
\\ \hline

Music ($90$,$1000$)
& $0.78482$ 
& $1.28709$ & $0.77347$ & $0.75646$ & $0.88779$ &  $0.79816$ & $0.76830$ & $-$ & 
$0.67777$ & $\underline{0.63486}$ & $0.78533$  \\ \hline


Telemonit ($19$, $1000$)
& $\underline{0.02872}$  
& $\underline{0.01491}$ & $0.65386$ & $0.84412$ & $0.02400$ & $5.71918$ & $0.86425$ & 
$-$ & $0.08053$ &
$0.08629$ & $0.94943$  \\ \hline

Forestfires($10$, $211$)
& $0.45773$ 
& $0.47749$ & $0.78057$ & $0.88979$ & $\underline{0.33891}$ & $0.37534$ & $0.96944$ 
& $\bf{0.17024}$ &
$0.47892$ & $0.51934$ & $1.05415$  \\ \hline

Propulsion ($15$,$200$) 
& $0.05832$ 
& $0.02341$ & $0.27768$ & $0.56418$ & $\underline{0.0129}$ & $\bf{0.00094}$ & $1.11210$ &
$0.01435$ & $0.01490$ & $0.02481$ & $10.2341$  \\ \hline

Brain ($29$,$300$)
& $0.97815$ & $\bf{2\textrm{e}-37}$ & $0.81711$ & $0.63700$ &
$\underline{5\textrm{e}-31}$ & $\underline{2\textrm{e}-6}$ & $0.89533$ &
$-$ &$\underline{4\textrm{e}-13}$& $0.00089$ & $1.04216$  \\ \hline

% rbfi  & \mfp & \si & \backf & \mars & \cosso & \spam &\addgp
%   & \lr & \lasso & \lar & &  \\

\hline
\hline
\end{tabular}
% \vspace{-0.1in}
\caption{ \small
The average squared error on the test set for all methods on 16 datasets.
% The dimensionality and number of training points is indicated next to the dataset.
% The best method(s) for each dataset are in bold. The second to fifth methods 
% are underlined. For the Speech dataset we have indicated the training time for
% each method.
% For \addkrrs we have also indicated the order $d$ chosen by our cross validation
% procedure in parantheses.
% The datasets with a * are actually lower dimensional datasets from the UCI repository. 
% But we
% artificially increase the dimensionality by inserting random values for the remaining
% coordinates. Even though, this doesn't change the function value it makes the
% regression problem harder.
}
\label{tb:realData}
}
\end{table}
% \end{sidewaystable}
\end{landscape}
}



==> _ <==

\newcommand{\insertTableReal}{
\newcommand{\tabletitlenumberspace}{-0.12in}
% \begin{sidewaystable}
\begin{landscape}
\begin{table}
{ %\footnotesize
\centering
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
% Dataset ($D$, $n$) & \addkrr & \krr & \ll & \lq & \svr & \gp & \backf  & \krr & \nw  \\
Dataset ($D$, $n$) & \addkrr & \krr & \knn & \nw & \locallin & \localquad 
  &\localcubic & \sveps &\svnu & \gp & \rt & \rbfi \\
\hline \\[\tabletitlenumberspace]
\hline 

Housing ($12$, $256$)& $\bf{0.26241}$ & $0.37690$ & $0.43620$ & $0.38431$ & 
  $\underline{0.31219}$ &
$\underline{0.35061}$ & $0.38528$ & $1.15272$ & $0.38600$ & $0.67563$ 
& $1.06015$ & $0.64871$  \\ \hline

Speech ($21$, $520$)& $\underline{0.02246} (2)$ & $0.03036$ & $0.09348$ & $0.11207$ & 
$0.03373$ &
$\underline{0.02404}$ & $0.02412$ & $0.22431$ & $0.06994$ & $0.02531$ & $0.05430$ & 
$0.03339$  \\ \hline

Music($400$, $90$)
& $0.92405$ (3) & $0.91458$ & $1.04258$ & $1.05745$ & $1.25804$ & $10.64825$ &
$904387.41462$ & $1.07009$ & $0.92568$ & $0.91722$ & $1.69992$ & $0.91248$  \\ \hline

Tele-total ($19$, $1000$)
& $\underline{0.03473}$ (9) & $0.05640$ & $0.09262$ & $0.21198$ & $0.08253$ & $0.18399$ &
$99.95821$ & $0.33902$ & $0.05246$ & $0.03948$ & $\bf{0.01375}$ &
$\underline{0.02872}$  \\ \hline

% Dataset ($D$, $n$) & \addkrr & \krr & \knn & \nw & \locallin & \localquad 
%   &\localcubic & \sveps &\svnu & \gp & \rt & \rbfi \\


\hline \\[-0.00in]
% \hline
 & \mfp & \si & \backf & \mars & \cosso & \spam &\addgp
  & \lr & \lasso & \lar & &  \\
\hline \\[\tabletitlenumberspace]
\hline 

Housing ($21$, $520$)& $0.38256$ & $0.50445$ & $0.64218$ & $0.42379$ & $1.30965$ &
$0.81653$ & $0.45656$ & $95.60708$ & $0.44515$ & $0.84410$  \\ \hline

Speech ($21$, $520$)& $0.02843$ & $0.39883$ & $0.36793$ & $\bf{0.01647}$ & $0.34863$ &
$0.66009$ & $-$ & $0.07392$ & $0.07303$ & $0.73916$  \\ \hline

% Tele-total ($19$, $1000$)
Music($400$, $90$)
& $1.49607$ & $1.10945$ & $1.06354$ & $1.79307$ & $4.24626$ & $1.09675$ & 
$-$ & $1.11007$ &
$0.90532$ & $1.12228$  \\ \hline

Tele-total ($19$, $1000$)
& $\underline{0.01491}$ & $\underline{0.65386}$ & $0.84412$ & $0.02400$ & $5.71918$ & $0.86425$ & 
$-$ & $0.08053$ &
$0.08629$ & $0.94943$  \\ \hline

%  & \mfp & \si & \backf & \mars & \cosso & \spam &\addgp
%   & \lr & \lasso & \lar & &  \\

\hline
\end{tabular}
\caption{ \small
The test set errors of all methods on 7 datasets from the UCI repository.
The dimensionality and number of training points is indicated next to the dataset.
The best method(s) for each dataset are in bold. \addkrrs performs best
in most of the datasets and is within the top 3 in all of the datasets.
In the Forest Fires dataset it is only slightly worse than \gp. In the
Propulsion dataset, \gps significantly outperforms all other methods.
}
\label{tb:realDataPres}
}
\end{table}
% \end{sidewaystable}
\end{landscape}
}



==> appProofs.tex <==

\section{Proof of Theorem~\ref{thm:zhangkrr}}
\label{sec:proofs}

We will be using the result of \citet{zhang13dividekrr} given in
Theorem~\ref{thm:zhangkrr}.
Note that the strategy will be choose $\lambda$ so as to balance the first two terms
in the RHS of the expression.

\begin{proof}[Proof of Theorem~\ref{thm:zhangkrr}]
\textbf{$\kernel_i$ is bounded and $\kernel$ times differentiable}:\\
First consider a product kernel $\kernelt = \kernel_1 \times \dots \kernel_d$.
If $\kernel_i$ is a $t$ times differentiable and bounded 
then the same could be said about $\kernelt$. For such kernels \citet{kuhn87eigvals}
(Theorem 4) gives us $\mu_j \leq C n^{-t/d -1}$ for some constant $C$.
Let the eigen expansion of $\kernelt$ be $\kernelt(x,x') = \sum_{j=1}^\infty 
\mut_j \phi_j(x) \phi_j(x')$.
Now, consider the kernel expansion of $\kernel = \sum_j \kernelj$ where each 
$\kernelj$ is $\kernelt$ on the group $\xj$. Since 
We set $\lambda = n^{-\frac{t+d}{t+2d}}$. 
Then,
\begin{align*}
\gamma(\lambda) = \sum_{j=1}^\infty \frac{1}{1 + \mu^{\kernelt}_j
  
\end{align*}


\end{proof}


==> expLong.tex <==
% \vspace{-0.06in}
\section{Experiments}
\label{sec:experiments}
% \vspace{-0.06in}

% \textbf{Alternatives for Comparison: } 
We compare \addkrrs to the following.
\textbf{Nonparametric models:} Kernel Ridge Regression (\krr),
$k$-Nearest Neighbors (\knn), 
Nadaraya Watson (\nw),
Locally Linear/ Quadratic interpolation (\locallin, \localquad),
$\epsilon$-Support Vector Regression (\sveps),
$\nu$-Support Vector Regression (\svnu),
Gaussian Process Regression (\gp),
Regression Trees (\rt),
Gradient Boosted Regression Trees (\gbrt) \cite{friedman00gbrt},
RBF Interpolation (\rbfi),
M5' Model Trees (\mfp) \citep{wang97m5prime}
and 
Shepard Interpolation (\si).
\textbf{Nonparametric additive Models:}
Back-fitting with cubic splines (\backf) \citep{hastie90gam},
Multivariate Adaptive Regression Splines (\mars) \citep{friedman91mars},
Component Selection and Smoothing (\cosso) \citep{lin03cosso},
Sparse Additive Models (\spam) \citep{ravikumar09spam}
and 
Additive Gaussian Processes (\addgp) \citep{duvenaud11additivegps}.
\textbf{Parametric models:}
Ridge Regression (\lr),
Least Absolute Shrinkage and Selection (\lasso) \cite{tibshirani94lasso} and
Least Angle Regression (\lar) \cite{efron04lar}.
We used software from 
\cite{chang11libsvm,jakabsons15regression,rasmussen06gps,lin03cosso,
hara13humanPose} or 
directly from Matlab. In some cases we used our own implementation.


% \vspace{-0.1in}
\subsection{Synthetic Experiments}
% \vspace{-0.05in}

We begin with a series of synthetic examples.
We compare \salsas to some non-additive methods to convey intuition about our additive
model.
% We compare only to subset of the above methods to avoid clutter in the figures.
We create a synthetic low order function of order $d=3$ in $D=15$ 
dimensions.
We do so first constructing the following $d$ dimensional function $f_d$ which
is the $\log$ of three Gaussian bumps,
  \begin{align*}
  f_d(x) = \log\Bigg(
    \alpha_1\frac{1}{h_d^d} \exp\left( \frac{\|x-v_1\|^2}{2h_d^2}
\right) + 
  \hspace{0.1in}  \alpha_1\frac{1}{h_d^d} 
      \exp\left( \frac{\|x-v_2\|^2}{2h_d^2} \right) + 
    (1-\alpha_1-\alpha_2)\frac{1}{h_d^d} \exp\left( \frac{\|x-v_3\|^2}{2h_d^2}
\right)
    \Bigg) \numberthis
  \label{eqn:fdtilde}
  \end{align*}
where $h_d = 0.01\sqrt{d}$, $\alpha_1,\alpha_2\in[0,1]$ and $v_i\in\RR^d$ are
constant vectors.
Then, we  add $f_d$ over all
${D\choose d}$ combinations of coordinates. We compare \addkrrs using order $3$ and
compare against others. The results are given in
Figure~\ref{fig:knownorder}.  
This setting is tailored to the assumptions of our method and, not surprisingly, it
outperforms all alternatives.

Next we demonstrate the bias variance trade-offs in using additive 
approximations 
on non-additive functions. We created a $15$ dimensional (non-additive) function and
fitted a \addkrrs model with $d = 1, 2, 4, 8, 15$ for difference
choices of $n$. The results are given in Figure~\ref{fig:comporder}.
The interesting observation here is that for small samples sizes small $d$ 
performs best. However, as we increase the sample size we can also increase the
capacity of the model by accommodating higher orders of interaction. In this regime,
large $d$ produces the best results. 
This illustrates our previous point that the
order of the additive model gives us another way to control the bias and variance
in a regression task.
We posit that when $n$ is extremely large,
$d=15$ will eventually  beat all other models.  
Finally, we construct synthetic functions in $D=20$
to $50$ dimensions and compare  against other methods in Figures~\ref{fig:cvone}
to~\ref{fig:cvfour}. Here, we chose $d$ via cross validation.
Our method outperforms or is competitive with other methods.
In these experiments, our function was $f_d$~\eqref{eqn:fdtilde} with $d=D$.

\insertFigToy

% \vspace{-0.05in}
\subsection{Real Datasets}
% \vspace{-0.1in}

Finally we compare \addkrrs against the other methods listed above on 16 datasets. The
datasets were taken from the UCI repository, Bristol Multilevel Modeling and 
the following sources: \citep{tegmark06lrgs,wehbe14brain,just10neurosemantic,
guillame14utility,tu14pancreatic,paschou07pca}.
Table~\ref{tb:realData} gives the average squared error on a test set.
% The dimensionality and number of training points is indicated next to the dataset.
The best method(s) for each dataset are in bold. The second to fifth methods 
are underlined. 
For the Speech dataset we have indicated the training time (including
cross validation for selecting hyper-parameters) for each method.
For \addkrrs we have also indicated the order $d$ chosen by cross validation.
% See the caption under the table for more details.
The datasets with a * are actually lower dimensional datasets from the UCI repository. 
But we
artificially increase the dimensionality by inserting random values for the remaining
coordinates. Even though, this doesn't change the function value it makes the
regression problem harder.
For all datasets, the test set was roughly the same size as the training set.

\addkrrs performs best (or is very close to the best) in 5 of the datasets.
Moreover it falls within the top $5$ in all but two datasets, coming sixth in both
instances. 
It is by far the most consistent of the 22 methods. 
% In the table we have also indicated the order $d$ of the \addkrrs model 
% chosen via cross validation. 

An interesting observation here is that
in many cases $d$ chosen by \salsas is much smaller than $D$, but \emph{importantly} 
also larger than $1$.
This observation (along with Fig~\ref{fig:comporder})
corroborates a key theme of this paper: while it is true that additive models 
improve the variance in high dimensional regression, it is often insufficient to
confine ourselves to just first order models.

\textbf{Some experimental details: }
\gps is the Bayesian interpretation of \krr. However, the results are
different in Table~\ref{tb:realData}. We believe this is due to differences in 
hyper-parameter tuning. For \gp, the 
GPML package~\cite{rasmussen06gps} optimises the
\gps marginal likelihood via L-BFGS. In contrast, our \krrs implementation
minimises the least squares cross validation error via grid search.
Some \addgps results are missing since it was very slow compared to 
other methods.
On the Blog dataset, \addkrrs took less than $35$s to train and all other
methods were completed in under 22 minutes. In contrast \addgps was not done training
even after several hours. Even on the relatively small speech dataset 
\addgps took about $80$ minutes.
Among the others, \backf, \mars, and \spams were the more expensive methods requiring
several minutes on datasets with large $D$ and $n$ 
whereas other methods took under 2-3 minutes.
We also experimented with locally cubic and quartic interpolation but exclude
them from the table since \locallin, \localquads generally performed better.



==> functionsel.tex <==

\subsection{Setting 2: Function Selection}

In this section, we study the ability of our method to recover 
the support of the true function.
We use RBF kernels on each group by setting kernel bandwidths
for each dimension as same as above.
Extending the generative model in \cite{ravikumar09spam}, 
we generate observations from the following
50-dimensional additive model:
\begin{align*}
	y_i =& f_1(x_{i1}) + f_2(x_{i2}) + f_3(x_{i3}) + f_4(x_{i4}) + \\
&f_1(x_{i5}x_{i6}) + f_2(x_{i7}x_{i8}) + \\
&f_3(x_{i9}x_{i10}) + f_4(x_{i11}x_{i12}) + \epsilon_i \\
f_1(x) =& -2\sin(2x), f_2(x) = x^2 - \frac{1}{3}, \\
f_3(x)=& x-\frac{1}{2}, f_4(x) = e^{-x} + e^{-1} - 1
\end{align*}
with noise $\epsilon_i \sim \mathcal{N}(0,1)$.
Thus, 46 out of 50 individual features are irrelevant, and
1221 out of 1225 pairwise features are irrelevant.

We then run our method where the component kernels
defined over all single dimensions and pairs of dimensions.
We plot the solution path for two independent datasets, 
with $n=200$ and $n=600$ observations, respectively.
Our results are shown in Figure \ref{fig:n200}.
With $n=600$ samples, at $\lambda=200$ we recover all true nonzero functions for a true positive rate of $100\%$ and have 47 false negatives for a false positive rate of $3.7\%$.

\begin{figure}
\centering
\includegraphics[width=3.4in]{figs/solnpath200.pdf}
\includegraphics[width=3.2in]{figs/solnpath600.pdf}
\vspace{\imcaptionspace}
\caption[]{\small Solution path with $n=200$ samples (above) and
$n=600$ (below). The $x$-axis shows the regularization parameter,
while the $y$-axis plots the $\ell_2$-norm of all $\beta_j$. The true nonzero functions are depicted in red.}
\vspace{\imtextspace}
\label{fig:n200}
\end{figure}



==> midExperiments.tex <==

\section{Experiments}
\label{sec:experiments}

\vspace{-0.1in}
We experimentally evaluate two criteria: the
performance of the different optimisation algorithms to minimise 
\eqref{eqn:optObjective}, and the performance of \addkrrs and other
nonparametric regression methods. 

% \subsubsection*{Experimental set up}
% \textbf{Experimental set up} \\
\textbf{Experimental set up} :
For our synthetic experiments, we take $\Xcal = [-1, 1]^D$.
We constructed a function of $3$ modes by taking the logarithm of $3$
Gaussian bumps whose centres are randomly chosen from $\Xcal$.
We uniformly randomly sample $500$ points each for training and testing from
$\Xcal$ and uses the true function values as the labels.
In the examples we consider below we take $D = 20$, $d = 4$ and $M = 50$. 
Therefore, our optimisation problem had $50 \times 500 = 25,000$ parameters.


% \subsubsection*{Comparison of Optimisation Algorithms}
% \textbf{Comparison of Optimisation Algorithms} \\
\textbf{Comparison of Optimisation Algorithms} :
We compared the five methods specified above on the synthetic example outlined
above. Figures~\ref{fig:iteration} and~\subref{fig:time} shows the improvement
in the objective over iterations and time respectively over $2000$ iterations. 
\subgrad and \proxgrad exhibit slow convergence but
\proxgradaccn, \bcdexact and \bcgddiag perform quite well. 
\proxgradaccn does marginally better than the rest.
Even for different values of $D$, $d$, $M$  we found that the latter three
methods did better but their relative performances varied slightly.
In our experiments below we use \proxgradaccn.

% \subsubsection*{Comparison with other Regression Algorithms}
% \textbf{Comparison with other Regression Algorithms} \\
\textbf{Comparison with other Regression Algorithms} :
We use the same experimental set up as explained above to compare \addkrrs
against the \krrs and \nws methods. To choose the kernel bandwidth for \nws  
we used $5$-fold cross validation. Due to time constraints, parameter selection 
 for \addkrrs and \krrs was very coarse -- we tried only $5$ different choices
for $(\lambda_1, \lambda_2)$ and used $2$-fold cross validation.
Despite this, \addkrrs significantly ourperforms both \krrs and \nws on the
synthetic problem. The results are depicted in Figure~\ref{fig:compare}. These
results are quite encouraging as they attest well to our intuitions about
favourable bias variance tradeoffs when using (statistically simpler) additive
models for high dimensional regression.

% \subsubsection*{Parkinson's Speech Dataset}
% \textbf{Parkinson's Speech Dataset}\\
\textbf{Parkinson's Speech Dataset} :
We compared \addkrr, \krrs and \nws on the above dataset from the UCI
repository. We used $21$ of the given features to predict the median pitch of
the speaker. The dataset had $1040$ instances, and we split them up equally for
training and testing. For \addkrrs we used $M = 50$, $d=4$. The test set errors
for \addkrr, \krrs and \nws were respectively $482.31$, $1071.80$ and
$1072.88$.
As before, \addkrrs outperforms other alternatives.

\begin{figure*}
\centering
\subfigure[]{
  \includegraphics[width=\imarrwthree]{figs/iteration2000v1} \hspace{\imhspthree}
  \vspace{\imlabelspace}
  \label{fig:iteration}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{figs/time2000v1} \hspace{\imhspthree}
  \vspace{\imlabelspace}
  \label{fig:time}
}
\subfigure[]{
  \includegraphics[width=\imarrwthree]{figs/toyResults}
  \vspace{\imlabelspace}
  \label{fig:compare}
} \\
\caption[]{ \hspace{-0.1in}
Figures~\subref{fig:iteration} and~\subref{fig:time} plot the objective value vs
iteration and cpu time respectively. Accelerated proximal gradient descent (blue
curve) seems to perform best. Figure~\subref{fig:compare} plots the test set
error for \addkrrs, \krrs and \nws on a synthetic problem. 
\addkrrs outperforms both methods.
}
\label{fig:toythree}
\vspace{\imtextspace}
\end{figure*}



==> optMethods.tex <==

\section{Optimisation Methods}
\label{sec:optMethods}

\subsubsection*{Subgradient Method}
Because our objective function is non-smooth, the simplest method is to solve it via 
the subgradient method. We implemented subgradient method with 
decreasing step sizes for our experiments. 
While subgradients can be computed cheaply in $O(nM)$, we observed poor 
convergence on our problem. %, as we would expect.

\subsubsection*{Proximal Gradient Method}

Note that we can write the objective \eqref{eqn:optObjective} as $F(\aalpha) =
G(\aalpha) + \Psi(\aalpha)$ where $G$ is smooth and $\Psi$ is not. $\Psi$ is the
popular group lasso penalty. Via the Moreau decomposition, and using the fact
that the argument in the prox operator is separable, the prox operator can
be shown to be,
\[
[\prox_{\Psi, t} (\aalpha)]^{(j)} =
\prox_{\Psi, t} (\alphaj) = 
  \begin{cases}
    \alphaj - t \frac{\alpha}{\|\alphaj\|_2} & \text{if } 
              \|\alphaj\| < t \\
    \zero & \text{otherwise}
  \end{cases}
\]
Obtaining the prox operator takes $O(nM)$ time and has cost comparable to
computing the gradient of $G(\aalpha)$. We use the above to implement proximal
gradient method as described in the class notes. We use backtracking to
determine the step size and experimented both with and without acceleration.

\subsubsection*{Exact Block Coordinate Descent via Newton trust region}

We can optimize the objective function over group $\alphaj$ with all other groups
$\alphai, i \ne j$ fixed. The objective is then
\[
\arg\min_\alphaj \frac{1}{2}\alphaj^T A_j \alphaj + b_j^T \alphaj + \lambda_2 \|\alphaj\|_2
\]
where $A_j = \KKj^T \KKj + \frac{\lambda_1}{2}\KKj$ 
and $b_j = -\KKj^T (y-\sum_{i\ne j}{\KKi \alphai}$.
This problem can be efficiently solved \citep{bcd-group-lasso:2013} 
by converting it to a one-dimensional trust-region problem. 
When $\|b_j\|_2 \le \lambda_2$, we have $\alphaj = 0$. 
Otherwise, there exists $t_j$ such that $\alphaj$ is the solution of
the following problem
\[
\arg\min_\alphaj \frac{1}{2}\alphaj^T A_j \alphaj + b_j^T \alphaj, 
\text{ such that } \|\alphaj\|_2 \le t_j.
\]
If $t_j$ is known we have $\alphaj = t_j * \left(-(t_j A_j + \lambda_2 I_n)^{-1} b_j\right)$
Because in this case $\|\alphaj\|_2 = t_j$, we have $\|(t_j A_j + \lambda_2 I_n)^{-1} b_j\|_2 = 1$.
As described in \citet{bcd-group-lasso:2013}, 
we can use Newton's method to solve this equation efficiently 
using the eigendecomposition of $A_j$, which is constant and needs to be computed only once.
However, this method does not scale well with $n$, since we still need
to solve an $n \times n$ linear system after $t_j$ is computed.
Thus, updating all blocks costs $O(n^3 M)$.

\subsubsection*{Block Coordinate Gradient Descent}

Because $\Psi(\aalpha)$, our $\ell_{1,2}$ group lasso penalty, is non-smooth yet block-separable,
we can apply the Coordinate Gradient Descent method \citep{cgd:2009}.
For each block of $\alphaj$, we solve
\[
\arg\min_{d_j} \frac{1}{2}d_j^T H_j d_j + \nabla_{j}G(\aalpha)^T d_j 
+ \lambda_2 \|\alphaj+d_j\|_2
\]
where $H_j \approx \nabla^2_{jj}G(\aalpha) = \KKj^T \KKj + \frac{\lambda_1}{2}\KKj$ 
and $\nabla_j G(\aalpha) = -\KKj^T (y-\sum_{i\ne j}{\KKi \alphai})$.
As suggested \citet{cgd:2009}, we use a diagonal matrix to approximate the true block Hessian.
We set $H_j = \max(\diag(\nabla^2_{jj}G(\aalpha))) I_n := h_j I_n$, so that a closed-form solution exists
for $d_j$:
\[
d_j = \frac{1}{h_j}\left(\lambda_2 \frac{\nabla_j G(\aalpha) - h_j \alphaj}
{\|\nabla_j G(\aalpha) - h_j \alphaj\|_2}\right).
\]
We use backtracking to determine the step size, then update $\alphaj \leftarrow \alphaj + t d_j$.

Because the Hessian is constant, each block update costs $O(n)$ and updating all blocks costs $O(nM)$.
Alternatively, as suggested in \citet{note-group-lasso:2010}, rather than using the 
diagonal Hessian approximation, we could approximately solve each block subproblem via 
coordinate descent.

